Graph Neural Network based scheduling : Improved throughput under a generalized interference model

In this work, we propose a Graph Convolutional Neural Networks (GCN) based scheduling algorithm for adhoc networks. In particular, we consider a generalized interference model called the $k$-tolerant conflict graph model and design an efficient approximation for the well-known Max-Weight scheduling algorithm. A notable feature of this work is that the proposed method do not require labelled data set (NP-hard to compute) for training the neural network. Instead, we design a loss function that utilises the existing greedy approaches and trains a GCN that improves the performance of greedy approaches. Our extensive numerical experiments illustrate that using our GCN approach, we can significantly ($4$-$20$ percent) improve the performance of the conventional greedy approach.

==> Max-k-Weighted Independent Set with Graph Convolutional Neural Networks/Results.tex <==
%\pgfplotstableread{./Results/K0_ER.csv} 
%\pgfplotstableread{./Results/K0_BA.csv} 
\section{Experiments}\label{section4}
We perform our experiments on a single GPU GeForce GTX 1080 Ti
\footnote{Training the models took around two hours.}.
The data used for training, validation and testing 
are described in the subsection below.
\subsection{Dataset}
\par We train our GCN using randomly generated graphs.
We consider two graph distributions, namely Erdos-Reyni (ER) and 
Barbasi-Albert (BA) models. These distributions were also used in \cite{9414098}. 
Our choice of these graph models is to ensure fair comparison with prior work 
on conflict graph model \cite{9414098} ($k=0$). 

In ER model with $N$ nodes, an edge is introduced between two nodes with 
a fixed probability $p$, independent of the generation of other edges. 
The BA model generates a graph with $N$ nodes (one node at a time),
preferentially attaching the node to $M$ existing nodes with probability 
proportional to the degree of the existing nodes. 
\par For training purpose, we generate $5000$ graphs of each of 
these models. For the ER model, we choose 
$p \in \{0.02, 0.05, 0.075, 0.10, 0.15\}$ and for the 
BA model we choose $M = Np$. The weights of the nodes are chosen 
uniformly at random from the interval $[0,1]$. We use an additional 
$50$ graphs for validation and $500$ graphs for testing.

\subsection{Choice of hyper-parameters}
We train a GCN with $3$ layers consisting i) an input layer 
with the weights of the nodes as input features
ii) a single hidden layer with $32$ features and 
iii) an output layer with $N$ features (one for each node)
indicating the likelihood of choosing the corresponding node in
the $k$-independent set. 
This choice of using a smaller number of layers ensures 
that the GCN operates with a minimal number of communications 
with its neighbors. We fix $k = 0$, and experiment training the GCN 
with different choices of the optimization weights $\beta_1$, $\beta_2$
and $\beta_3$. The results obtained are tabulated in Figure \ref{fig:table1}. Let $W_{gr}$ denote the total weight of 
the plain greedy algorithm i.e., without any GCN and $W_{gcn}$ 
denote the total weight of the independent set predicted by the
GCN-greedy combination. We have tabulated the average ratio 
between the total weight of the nodes in the independent set 
obtained from the GCN-greedy and the total weight 
of the nodes in the independent set obtained from the plain greedy algorithm, i.e., $W_{gcn}/W_{gr}$. The average is taken over the 
test data set.
\begin{figure}
\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c|c| } 
\hline
 & & & & \multicolumn{2}{c|}{Test Data = ER} &  
 \multicolumn{2}{c|}{Test Data = BA}  \\ \cline{5-8} 
Training Data & $\beta_1$ & $\beta_2$ & $\beta_3$ & Average & Variance & Average & Variance \\
& & & &$W_{gcn}/W_{gr}$ & $\times \; 10^{-3}$ & $W_{gcn}/W_{gr}$& $\times \; 10^{-3}$  \\
\hline
\multirow{8}{*}{BA} &	5	&	5	&	10	&	1.038 	&	3.047
	&	1.11 & 10.16	\\
&	10	&	10	&	1	&   1.035 	&	3.297 &	 1.11	&	10.37	\\
&	5	&	5	&	1	&	1.035 	&	3.290 &	1.11	&	10.14	\\
&	1	&	1	&	1	&	1.034 	&	3.253	&	1.10	&	10.23	\\
&	5	&	5	&	30	&	1.041 	&	3.230	&	1.10	&	10.39	\\
&	5	&	5	&	50	&	1.041 	&	3.214 &	1.10	&	10.28	\\
&	5	&	5	&	100	&	1.035 	&	2.838 &	1.09	&	10.02	\\
&	30	&	1	&	1	&	1.031 	&	2.401 &	1.07	&	8.25	\\
 \hline
\multirow{8}{*}{ER} & 5 & 5 & 30 & 1.040 & 2.929
& 1.10	&	10.12 \\
 & 5 & 5 & 10 & 1.039 & 3.145 &
1.11	&	10.71	\\
 & 5 & 5 & 50 & 1.039 & 2.957 &
1.09	&	9.92 \\ 
 &	1	&	1	&	1	&	1.038 	&	3.135	&	1.11	&	10.74 \\
&	1	&	20	&	1	&	1.036 	&	3.070	&	1.11	&	10.55 \\
&	10	&	10	&	1	&	1.034 	&	3.428	&	1.11	&	10.34 \\
&	5	&	5	&	1	&	1.034 	&	3.331	&	1.11	&	10.34\\
&	5	&	5	&	100	&	1.031 	&	2.420	&	1.08	&	8.42\\
 \hline
 \multicolumn{4}{|c|}{Distributed scheduling using GNN 
 \cite{9414098}} & 1.039 & 3.5 & 1.11 & 11.0 \\
 \hline
\end{tabular}
\caption{Table showing the average and variance of the ratio of the total 
weight of the nodes in the independent set ($K=0$) obtained using GCN to 
that of the independent set obtained using greedy algorithm. 
We observe a $3$ percent increase in the total weight for the ER model and 
$11$ percent increase in the total weight for the BA model. 
Our performance matches with the performance of the GCN used in
\cite{9414098}.}
\vspace{-1.5em}
\label{fig:table1}
\end{center}
\end{figure}
The training was done with BA and ER models separately. We test 
the trained models also with test data from both models to understand if the trained models are transferable. 
We see that GCN trained with  
parameters $\beta_1 = 5$, $\beta_2 = 5$ and $\beta_3 = 10$
performs well 
for both ER and BA graph models. 
The GCN improves the total weight of the 
greedy algorithm by $4$ percent for the ER model and 
by $11$ percent for the BA model.
Also, we see that the GCN trained with ER
model performs well with BA data and vice versa.  

\subsection{Performance for different $k$}
We also evaluate the performance for different tolerance values
$k \in \{1,2,3,4\}$. We use the parameters 
$\beta_1 = 5$, $\beta_2 = 5$ and $\beta_3 = 10$ 
in the cost function. Recall that we have come up with this 
choice using extensive simulations for $k=0$.
In Figure~\ref{fig:table2}, we tabulate the average ratio 
between the total weight of the $k$-independent set obtained 
using the GCN-greedy combo and that of the plain greedy algorithm
i.e., $W_{gcn}/W_{gr}$. 
We have also included the variance from this performance. 
We observe that the performance for a general $k$ is even better 
as compared to $k=0$. For example, we see that for $k = 2,3,4$, 
we see  $6$ percent improvement for the ER model and close to $20$
percent improvement for the BA model.
\begin{figure}
\begin{center}
\begin{tabular}{ |c|c|c|c|c|c| } 
\hline
 & & \multicolumn{2}{c|}{Test Data = ER} &  
 \multicolumn{2}{c|}{Test Data = BA}  \\ \cline{3-6} 
Training Data & $k$ & Average & Variance & Average & Variance \\
& &$W_{gcn}/W_{gr}$ & $\times \; 10^{-3}$ & $W_{gcn}/W_{gr}$& $\times \; 10^{-3}$  \\
\hline
    \multirow{4}{*}{BA} &	1	&	1.056	&	4.07	&	1.143	&	10.22	\\
&	2	&	1.062	&	5.26	&	1.193	&	10.92	\\
&	3	&	1.067	&	5.55	&	1.209	&	20.14	\\
&	4	&	1.063	&	4.53	&	1.241	&	20.57	\\
\hline
\multirow{4}{*}{ER} &	1	&	1.056	&	3.99	&	1.143	&	10.18	\\
&	2	&	1.064	&	5.12	&	1.187	&	10.81	\\
&	3	&	1.066	&	4.82	&	1.205	&	20.13	\\
&	4	&	1.062	&	4.18	&	1.225	&	20.29	\\
 \hline
\end{tabular}
\caption{The table shows the average and variance of the 
ratio between the total weight of the $k$-independent set obtained using GCN-greedy combo to that of the plain greedy algorithm for $k \in \{1,2,3,4\}$. We observe that the improvement is consistently 
above $5$ percent for the ER model and above $14$ percent 
for the BA model.}
\vspace{-1.5em}
\label{fig:table2}
\end{center}
\end{figure}

Interestingly, the GCN trained with ER graphs performs well on 
the BA data set as well. This indicates that the trained GCN
is transferable to other models. 


\begin{comment}
\begin{figure}[t!]
   \centering
  %  \begin{tabular}{c}
   %        \multirow{8}{*}{BA} \\
    %       \multirow{8}{*}{ER} 
     %   \end{tabular}%
\begin{subfigure}[t]{0.5\textwidth}
\centering
\pgfplotstabletypeset[col sep=comma,
%every column no 0/.append style={before column=
%\multirow{8}{*}{BK}},
columns={Model,b1,b2,b3,avg,var},
columns/Model/.style={string type, column name = Training  Data},
every head row/.style={before row=\hline,after row=\hline},	% style the first row
	every last row/.style={after row=\hline},	% style the last row
%	every first column/.style={column type/.add={|}{}},	
	every column/.style={column type/.add={|}{}},	
	every last column/.style={column type/.add={}{|}},
columns/b1/.style={column name = $\beta_1$}, 
columns/b2/.style={column name = $\beta_2$}, 
columns/b3/.style={column name = $\beta_3$},
columns/avg/.style={column name = Average, precision=3},
columns/var/.style={column name = Variance, precision=3}
] {./Results/K0_ER.csv}
    \caption{Caption}
    \label{fig:my_label}
\end{subfigure}%
\begin{subfigure}[t]{0.5\textwidth}
\centering
\pgfplotstabletypeset[col sep=comma,
columns={b1,b2,b3,avg,var},
%columns/Model/.style={string type, column name = Training  Data},
every head row/.style={before row=\hline,after row=\hline},	% style the first row
	every last row/.style={after row=\hline},	% style the last row
%	every first column/.style={column type/.add={|}{}},	
	every column/.style={column type/.add={|}{}},	
	every last column/.style={column type/.add={}{|}},
columns/b1/.style={column name = $\beta_1$}, 
columns/b2/.style={column name = $\beta_2$}, 
columns/b3/.style={column name = $\beta_3$},
columns/avg/.style={column name = Average},
columns/var/.style={column name = Variance}] {./Results/K0_BA.csv}
    \caption{Caption}
    \label{fig:my_label}
    \end{subfigure}
\end{figure}
\end{comment}


==> Max-k-Weighted Independent Set with Graph Convolutional Neural Networks/figure1.tex <==
\begin{figure}[h]
\begin{center}
\scalebox{0.8}{
\begin{tikzpicture}
\tikzstyle{state}=[shape=circle,draw,minimum size=0.5cm,fill=darkolivegreen!50]
%[scale=.9,auto=center,every node/.style={circle,fill=darkolivegreen!50}]

\node[state] (a1) at (1,2){U1};
\node[state] (a2) at (4,2.5){U2};
\node[state] (a3) at (1.5,-0.5){U3};
\node[state] (a4) at (4.5,-1){U4};
\node[state] (a5) at (5,1){U5};

\path[-,draw,thick]
(a1) edge node[midway,above, rotate=0] {$l_{12}$} (a2)
(a2) edge node[midway,above, rotate = 45] {$l_{23}$} (a3)
(a2) edge node[midway,below,rotate=135] {$l_{25}$} (a5)
% (a1) edge node[midway,above] {$l_{16}$} (a6)
% (a3) edge node[midway,above] {$l_{36}$} (a6)
% (a4) edge node[midway,above] {$l_{46}$} (a6)
(a3) edge node[midway,above,rotate=0] {$l_{35}$} (a5)
(a4) edge node[midway,above,rotate=80] {$l_{45}$} (a5)
(a1) edge node[midway,above,rotate=125] {$l_{13}$} (a3)
(a3) edge node[midway,above,rotate=0] {$l_{34}$} (a4);

\draw[->] (6,1) -- (9,1) node[midway,below] {$k$-tolerant conflict graph};
%\node[above] {$l_12$};

\node[state] (a6) at (10,1.8){$l_{13}$};
\node[state] (a7) at (11,3){$l_{12}$};
\node[state] (a8) at (13,3){$l_{23}$};
\node[state] (a9) at (12,1.5){$l_{25}$};
\node[state] (a10) at (11.5,-0.5){$l_{35}$};
\node[state] (a11) at (14,0){$l_{34}$};
\node[state] (a12) at (14.2,1){$l_{45}$};

\draw (a6) -- (a7);
\draw (a6) -- (a10);
\draw (a7) -- (a8);
\draw (a7) -- (a9);
\draw (a8) -- (a9);
\draw (a9) -- (a12);
\draw (a10) -- (a11);
\draw (a9) -- (a10);
\draw (a11) -- (a12);
\draw (a10) -- (a12);
\end{tikzpicture}}\\
\caption{Graph representation of a wireless multi-hop network ($U_i$'s denote the users in the network and $l_{ij}$ denotes the link between the users $U_i$ and $U_j$) with its $k$-tolerant conflict graph model}
\label{fig:wireless_network_graph}
\end{center}
\end{figure}

==> Max-k-Weighted Independent Set with Graph Convolutional Neural Networks/figure21.tex <==
\begin{figure}[h]
\begin{center}
\scalebox{0.8}{
\begin{tikzpicture}
\tikzstyle{state}=[shape=circle,draw,minimum size=0.5cm,fill=darkolivegreen!50]
%[scale=.9,auto=center,every node/.style={circle,fill=darkolivegreen!50}]

\node[state] (a1) at (1,2){U1};
\node[state] (a2) at (4,2.5){U2};
\node[state] (a3) at (1.5,-0.5){U3};
\node[state] (a4) at (4.5,-1){U4};
\node[state] (a5) at (5,1){U5};

\path[-,draw,thick]
(a1) edge node[midway,above, rotate=0] {$l_{12}$} (a2)
(a2) edge node[midway,above, rotate = 45] {$l_{23}$} (a3)
(a2) edge node[midway,below,rotate=135] {$l_{25}$} (a5)
% (a1) edge node[midway,above] {$l_{16}$} (a6)
% (a3) edge node[midway,above] {$l_{36}$} (a6)
% (a4) edge node[midway,above] {$l_{46}$} (a6)
(a3) edge node[midway,above,rotate=0] {$l_{35}$} (a5)
(a4) edge node[midway,above,rotate=80] {$l_{45}$} (a5)
(a1) edge node[midway,above,rotate=125] {$l_{13}$} (a3)
(a3) edge node[midway,above,rotate=0] {$l_{34}$} (a4);

\draw[->] (6,1) -- (9,1) node[midway,below] {$k$-tolerant conflict graph};
%\node[above] {$l_12$};

\node[state] (a6) at (10,1.8){$l_{13}$};
\node[state] (a7) at (11,3){$l_{12}$};
\node[state] (a8) at (13,3){$l_{23}$};
\node[state] (a9) at (12,1.5){$l_{25}$};
\node[state] (a10) at (11.5,-0.5){$l_{35}$};
\node[state] (a11) at (14,0){$l_{34}$};
\node[state] (a12) at (14.2,1){$l_{45}$};

\draw (a6) -- (a7);
\draw (a6) -- (a10);
\draw (a7) -- (a8);
\draw (a7) -- (a9);
\draw (a8) -- (a9);
\draw (a9) -- (a12);
\draw (a10) -- (a11);
\draw (a9) -- (a10);
\draw (a11) -- (a12);
\draw (a10) -- (a12);
\end{tikzpicture}}\\
\caption{Graph representation of a wireless multi-hop network ($U_i$'s denote the users in the network and $l_{ij}$ denotes the links between the users $U_i$ and $U_j$) with its $k$-tolerant conflict graph model}
\label{fig:wireless_network_graph}
\end{center}
\end{figure}

==> figure1.tex <==
\begin{figure}[h]
\begin{center}
\scalebox{0.8}{
\begin{tikzpicture}
\tikzstyle{state}=[shape=circle,draw,minimum size=0.5cm,fill=darkolivegreen!50]
%[scale=.9,auto=center,every node/.style={circle,fill=darkolivegreen!50}]

\node[state] (a1) at (1,2){U1};
\node[state] (a2) at (4,2.5){U2};
\node[state] (a3) at (1.5,-0.5){U3};
\node[state] (a4) at (4.5,-1){U4};
\node[state] (a5) at (5,1){U5};

\path[-,draw,thick]
(a1) edge node[midway,above, rotate=0] {$l_{12}$} (a2)
(a2) edge node[midway,above, rotate = 45] {$l_{23}$} (a3)
(a2) edge node[midway,below,rotate=135] {$l_{25}$} (a5)
% (a1) edge node[midway,above] {$l_{16}$} (a6)
% (a3) edge node[midway,above] {$l_{36}$} (a6)
% (a4) edge node[midway,above] {$l_{46}$} (a6)
(a3) edge node[midway,above,rotate=0] {$l_{35}$} (a5)
(a4) edge node[midway,above,rotate=80] {$l_{45}$} (a5)
(a1) edge node[midway,above,rotate=125] {$l_{13}$} (a3)
(a3) edge node[midway,above,rotate=0] {$l_{34}$} (a4);

\draw[->] (6,1) -- (9,1) node[midway,below] {$k$-tolerant conflict graph};
%\node[above] {$l_12$};

\node[state] (a6) at (10,1.8){$l_{13}$};
\node[state] (a7) at (11,3){$l_{12}$};
\node[state] (a8) at (13,3){$l_{23}$};
\node[state] (a9) at (12,1.5){$l_{25}$};
\node[state] (a10) at (11.5,-0.5){$l_{35}$};
\node[state] (a11) at (14,0){$l_{34}$};
\node[state] (a12) at (14.2,1){$l_{45}$};

\draw (a6) -- (a7);
\draw (a6) -- (a10);
\draw (a7) -- (a8);
\draw (a7) -- (a9);
\draw (a8) -- (a9);
\draw (a9) -- (a12);
\draw (a10) -- (a11);
\draw (a9) -- (a10);
\draw (a11) -- (a12);
\draw (a10) -- (a12);
\end{tikzpicture}}\\
\caption{Graph representation of a wireless multi-hop network ($U_i$'s denote the users in the network and $l_{ij}$ denotes the link between the users $U_i$ and $U_j$) with its $k$-tolerant conflict graph model}
\label{fig:wireless_network_graph}
\end{center}
\end{figure}

==> figure21.tex <==
\begin{figure}[h]
\begin{center}
\scalebox{0.8}{
\begin{tikzpicture}
\tikzstyle{state}=[shape=circle,draw,minimum size=0.5cm,fill=darkolivegreen!50]
%[scale=.9,auto=center,every node/.style={circle,fill=darkolivegreen!50}]

\node[state] (a1) at (1,2){U1};
\node[state] (a2) at (4,2.5){U2};
\node[state] (a3) at (1.5,-0.5){U3};
\node[state] (a4) at (4.5,-1){U4};
\node[state] (a5) at (5,1){U5};

\path[-,draw,thick]
(a1) edge node[midway,above, rotate=0] {$l_{12}$} (a2)
(a2) edge node[midway,above, rotate = 45] {$l_{23}$} (a3)
(a2) edge node[midway,below,rotate=135] {$l_{25}$} (a5)
% (a1) edge node[midway,above] {$l_{16}$} (a6)
% (a3) edge node[midway,above] {$l_{36}$} (a6)
% (a4) edge node[midway,above] {$l_{46}$} (a6)
(a3) edge node[midway,above,rotate=0] {$l_{35}$} (a5)
(a4) edge node[midway,above,rotate=80] {$l_{45}$} (a5)
(a1) edge node[midway,above,rotate=125] {$l_{13}$} (a3)
(a3) edge node[midway,above,rotate=0] {$l_{34}$} (a4);

\draw[->] (6,1) -- (9,1) node[midway,below] {$k$-tolerant conflict graph};
%\node[above] {$l_12$};

\node[state] (a6) at (10,1.8){$l_{13}$};
\node[state] (a7) at (11,3){$l_{12}$};
\node[state] (a8) at (13,3){$l_{23}$};
\node[state] (a9) at (12,1.5){$l_{25}$};
\node[state] (a10) at (11.5,-0.5){$l_{35}$};
\node[state] (a11) at (14,0){$l_{34}$};
\node[state] (a12) at (14.2,1){$l_{45}$};

\draw (a6) -- (a7);
\draw (a6) -- (a10);
\draw (a7) -- (a8);
\draw (a7) -- (a9);
\draw (a8) -- (a9);
\draw (a9) -- (a12);
\draw (a10) -- (a11);
\draw (a9) -- (a10);
\draw (a11) -- (a12);
\draw (a10) -- (a12);
\end{tikzpicture}}\\
\caption{Graph representation of a wireless multi-hop network ($U_i$'s denote the users in the network and $l_{ij}$ denotes the links between the users $U_i$ and $U_j$) with its $k$-tolerant conflict graph model}
\label{fig:wireless_network_graph}
\end{center}
\end{figure}
